Two Simple Ways to Learn Individual Fairness Metrics from Data

Individual fairness is an intuitive definition of algorithmic fairness that addresses some of the drawbacks of group fairness. Despite its benefits, it depends on a task specific fair metric that encodes our intuition of what is fair and unfair for the ML task at hand, and the lack of a widely accepted fair metric for many ML tasks is the main barrier to broader adoption of individual fairness. In this paper, we present two simple ways to learn fair metrics from a variety of data types. We show empirically that fair training with the learned metrics leads to improved fairness on three machine learning tasks susceptible to gender and racial biases. We also provide theoretical guarantees on the statistical performance of both approaches.

==> VIML.tex <==
\section{VIML: A Variational Inequality approach to Metric Learning}
\label{eq:VIML}

The standard approach to fitting \eqref{eq:binaryResponseModel} is maximum likelihood. Unfortunately, except for certain special choices of $F_0$ (\eg\ the logistic function), the log-likelihood is not concave:
\begin{equation}
\begin{aligned}
\ell_n(\Sigma) &= \frac1n\sum_{i=1}^ny_i\log\frac{F_0(-\langle D_i,\Sigma\rangle)}{1-F_0(-\langle D_i,\Sigma\rangle)} \\
&\quad+ \log(1-F_0(-\langle D_i,\Sigma\rangle)).
\end{aligned}
\label{eq:log-likelihood}
\end{equation}
To avoid this issue, we consider a variational inequality (VI) approach: find $\hSigma\in\symm_+^d$ such that 
\begin{equation}
\begin{aligned}
\langle M_n(\hSigma),\Sigma - \hSigma\rangle \ge 0\text{ for all }\Sigma\in\symm_+^d, \\\textstyle
M_n(\Sigma) \triangleq \frac1n\sum_{i=1}^n(y_i - F_0(-\langle D_i,\Sigma\rangle))D_i.
\end{aligned}
\label{eq:VIML}
\end{equation}
It is not obvious why \eqref{eq:VIML} is a good estimator of $\Sigma_0$, but, as we shall see, $\Sigma_0$ is the unique symmetric matrix that satisfies
\[
\begin{aligned}
\langle M(\Sigma_0),\Sigma - \Sigma_0\rangle \ge 0\text{ for all }\Sigma\in\symm_+^d, \\
M(\Sigma) \triangleq \Ex\big[(y_i - F_0(-\langle D_i,\Sigma\rangle))D_i\big].
\end{aligned}
\]
The main benefit of estimating $\Sigma_0$ with \eqref{eq:VIML} is computational. As long as $F_0$ is non-increasing, it is not hard to see that $M_n:\symm^d\to\symm^d$ is \emph{monotone}:
\[
\begin{aligned}
&\langle M_n(\Sigma_1) - M_n(\Sigma_2), \Sigma_1 - \Sigma_2\rangle \\
% &\quad = \frac1n\sum_{i=1}^n(F_0(-\langle D_i,\Sigma_2\rangle) - F_0(-\langle D_i,\Sigma_1\rangle))\langle D_i,\Sigma_1 - \Sigma_2\rangle \\
&\quad = \frac1n\sum_{i=1}^n(F_0(-\langle D_i,\Sigma_2\rangle) - F_0(-\langle D_i,\Sigma_1\rangle))(\langle D_i,\Sigma_1 - \Sigma_2\rangle) \\
&\quad\ge 0,
\end{aligned}
\]
where the second step is a consequence of the monotonicity of $F_0$. Thus \eqref{eq:VIML} is a monotone VI problem, which is efficiently solvable by  first-order methods. In the rest of this section, we describe two how to solve \eqref{eq:VIML} efficiently.

Two common families of methods for solving monotone VI problems are gradient-type methods \cite{bruck1977weak} and extra-gradient-type methods \cite{korpelevich1976extragradient}. We adopt standard notation for a VI problem: find $x_*\in C$ such that
\begin{equation}
\langle G(x_*),x-x_*\rangle \ge 0\text{ for all }x\in C.
\label{eq:VI}
\end{equation}
Gradient-type methods generate a sequence of iterates by the update rule
\[
x_{t+1} \gets P_C(x_t - \eta_tG(x_t)),
\]
where $\eta_t > 0$ is a step size parameter. The iterates are guaranteed to converge if $G$ is \emph{strongly-monotone}, but may oscillate if $F$ is not strongly monotone \cite{gidel2018Variational}. It is possible to stabilize the iterates of gradient-type methods by averaging the iterates, but the average converges slowly to a solution \cite{nedic2009Subgradient}. 

On the other hand, extra-gradient methods do not depend on averaging to converge to a solution (even in cases where gradient-type methods fail to converge). They generate a sequence of iterates by the update rule
\begin{equation}
\begin{aligned}
x_{t+\frac12} \gets P_C(x_t - \eta_tG(x_t)), \\
x_{t+1} \gets P_C(x_t - \eta_tG(x_{t+\frac12})).
\end{aligned}
\label{eq:extraGradientUpdate}
\end{equation}
The idea of the extra-gradient method is to using a look-ahead step to approximate the backward/implicit update rule \cite{gidel2018Variational}: 
\begin{equation}
x_{t+1} \gets P_C(x_t - \eta_tG(x_{t+1})).
\label{eq:implicitUpdate}
\end{equation}
Backward/implicit methods based on \eqref{eq:implicitUpdate} more stable than their forward/explicit counterparts, but they are usually not practical due to the cost of evaluating \eqref{eq:implicitUpdate}. This idea of stabilizing a method by evaluating the gradient at an extrapolated point is more generally known as \emph{extrapolation} in mathematical optimization and pre-dates Korpelevich's work. 

For large-scale problems (including the applications we consider in Section \ref{sec:computationalResults}), vanilla (batch) gradient-type and extra-gradient-type methods are too expensive, and we consider their stochastic counterparts instead. The stochastic gradient update rule is 
\[
x_{t+1} \gets P_C(x_t - \eta_tG_t),
\]
where $G_t$ is an unbiased estimate of $G(x_t)$, and the stochastic extra-gradient (SEG) update rule is 
\[
\begin{aligned}
x_{t+\frac12} \gets P_C(x_t - \eta_t(G_t)), \\
x_{t+1} \gets P_C(x_t - \eta_tG_{t+\frac12}).
\end{aligned}
\]
For both methods, we average the iterates 
\begin{equation}
\bar{x}_t \triangleq \frac{\sum_{s=1}^t\eta_sx_s}{\sum_{s=1}^t\eta_s}
\label{eq:averaging}
\end{equation}
to obtain a convergent sequence. It is possible to compute the average iterate online:
\[
\begin{aligned}
\bar{x}_t &= \frac{\eta_t}{\sum_{s=1}^t\eta_t}x_t + \frac{\sum_{s=1}^{t-1}\eta_t}{\sum_{s=1}^t\eta_t}\bar{x}_{t-1} \\
&\triangleq \bar{\eta}_tx_t + (1 - \bar{\eta}_t)\bar{x}_{t-1}
\end{aligned}
\]
For instance, letting $\bar{\eta}_t = \frac1t$ is uniform averaging ($\eta_t = 1$), while letting $\bar{\eta}_t = 1-\beta$ for some $\beta\in(0,1)$ is geometric averaging ($\eta_t = \beta^{T-t}$). 
% We study the convergence rates of both methods in subsection \ref{sec:computationalTheory}.

% We summarize the two methods in Algorithms .

% \begin{algorithm}[tb]
% \caption{stochastic gradient method}
% \label{alg:SG}
% \begin{algorithmic}
%   \State {\bfseries Input:} starting point $x_*$, step sizes $(\eta_t)$
%   \Repeat
%     \State $x_{t+1} \gets P_C(x_t - \eta_tG_t)$,
%   \Until{converged}
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[tb]
% \caption{stochastic extra-gradient method}
% \label{alg:SEG}
% \begin{algorithmic}
%   \State {\bfseries Input:} starting point $x_*$, step sizes $(\eta_t)$
%   \Repeat
%     \State $x_{t+\frac12} \gets P_C(x_t - \eta_t(G_t))$
%     \State $x_{t+1} \gets P_C(x_t - \eta_tG_{t+\frac12})$
%   \Until{converged}
% \end{algorithmic}
% \end{algorithm}

==> computationalTheory.tex <==
\subsection{Computational theory}
\label{sec:computationalTheory}

In this section, we study the convergence rates of the stochastic gradient and stochastic extra-gradient (SEG) methods for solving \eqref{eq:VIML}. We measure the quality of an iterate $x$ with a \emph{merit function}: a function $\varphi:C\to\reals_+$ such that $\varphi(x) = 0$ if and only if $x$ satisfies \eqref{eq:VI}. A typical metric function for VI problems in which $G$ is continuous and $C$ is bounded is
\begin{equation}
\varphi(x) = \sup_{y\in C}\langle G(y),x - y\rangle.
\label{eq:meritFunction}
\end{equation}
It is not hard to see that $\varphi(x^*) = 0$ if and only if $x^*$ satisfies a weak form of \eqref{eq:VI}:
\begin{equation}
\langle G(x),x-x_*\rangle \ge 0\text{ for all }x\in C.
\label{eq:weakVI}
\end{equation}
As long as $F$ is continuous, \eqref{eq:weakVI} and \eqref{eq:VI} are equivalent, so $\varphi(x^*) = 0$ if and only if $x^*$ satisfies \eqref{eq:VI}. 

One issue with \eqref{eq:meritFunction} VI problems with unbounded feasible sets is its value may be infinite. To avoid this issue, it is standard to modify the merit function by restricting the sup in \eqref{eq:meritFunction} to a bounded subset of the feasible set:
\begin{equation}
\varphi_r(x) = \sup_{y\in C:\|y - x_*\|\le R}\langle G(y),x - y\rangle.
\label{eq:restrictedMeritFunction}
\end{equation}
There are no restrictions on $x_*\in C$ in \eqref{eq:restrictedMeritFunction}, but $R > 0$ must be large enough so that $\{x\in C:\|x - x_*\|\le R\}$ contains a solution to the VI problem. If \eqref{eq:restrictedMeritFunction} is used to measure the progress of an iterative method for solving the VI problem, then $x_*$ is usually the initial iterate, and $R$ is an upper bound on the distance to the closest solution. It is not hard to see that \eqref{eq:restrictedMeritFunction} is a valid merit function for the restricted VI problem: $x^*\in C_R(x_*) \triangleq \{x\in C:\|x - x_*\| \le R\}$ such that
\begin{equation}
\langle G(x_*),x-x_*\rangle \ge 0\text{ for all }x\in C_R(x_*)
\label{eq:VI}
\end{equation}

We check that \eqref{eq:restrictedMeritFunction} also certifies $x^*$ is a solution of the (unrestricted) VI \eqref{eq:VI}.

\begin{lemma}
\label{lem:restrictedMeritFunction}
If $\varphi(x^*) = 0$ and $\|x^* - x_*\| < R$, then $x^*$ satisfies \eqref{eq:VI}.
\end{lemma}

In the rest of this subsection, we measure the progress of the stochastic gradient and SEG methods with \eqref{eq:restrictedMeritFunction}. First, we study the convergence rate of the SEG method because it converges under more general conditions that the stochastic gradient method. 

\begin{assumption}
\label{asm:Lipschitz}
The map $F$ is $L$-Lipschitz: 
\[
\|G(x_1) - G(x_2)\| \le L\|x_1 - x_2\|\text{ for all }x_1,x_2\in C.
\]
\yk{Assumption 4.3 implies this}
\end{assumption}

\begin{assumption}
\label{asm:boundedVariance}
The variance of $G_t$ is bounded: 
\[
\sigma^2 \triangleq \Ex_t\big[\|G_t - G(x_t)\|^2\big] < \infty\text{ for all }t.
\]
\end{assumption}

\begin{theorem}
\label{thm:SEGconvergenceRate}
Under Assumptions \ref{asm:Lipschitz} and \ref{asm:boundedVariance}, as long as $R > \|x^* - x_*\|$, the SEG method with a constant step size  $\eta_t = \eta\triangleq \frac{1}{\sqrt{3}L}$ and uniform averaging satisfies
\[
\varphi(\bar{x}_T) \le \frac{R}{\eta T} + \frac72\eta\sigma^2\text{ for all }T.
\]
\end{theorem}

\begin{corollary}
Under the conditions of Theorem \ref{thm:SEGconvergenceRate}, picking $\eta = (\frac{2R}{7\sigma^2T})^{\frac12}$ leads to $\varphi(\bar{x}_T) \le (\frac{7R\sigma^2}{2T})^{\frac12}$.
\end{corollary}

To show the stochastic gradient method converges, we need another assumption.

\begin{assumption}
\label{asm:boundedGradient}
The map $G$ is bounded: $\|G(x)\|_2 \le B$ for all $x\in C$.
\yk{Assumption 4.1 implies this}
\end{assumption}

\begin{theorem}
\label{thm:SGconvergenceRate}
Under Assumptions \ref{asm:Lipschitz}, \label{asm:boundedGradient}, and \ref{asm:boundedVariance}, as long as $R > \|x^* - x_*\|$, the SG method with a constant step size  $\eta_t = \eta$ and uniform averaging satisfies
\[
\varphi(\bar{x}_T) \le \frac{R}{2\eta T} + \frac{B^2 + \sigma^2}{2}\eta\text{ for all }T.
\]
\end{theorem}

\begin{corollary}
Under the conditions of Theorem \ref{thm:SEGconvergenceRate}, picking $\eta = (\frac{2R}{7\sigma^2T})^{\frac12}$ leads to $\varphi(\bar{x}_T) \le (\frac{7R\sigma^2}{2T})^{\frac12}$.
\end{corollary}

==> data_prep.tex <==
\section{Bios data preparation}

We follow the approach of \citep{de2019bias}\footnote{\url{https://github.com/microsoft/biosbias}} to collect biographies from the internet, where we select 4 occupations highly susceptible to gender biases: attorney, paralegal, physician and nurse. As class paralegal is relatively rare (only 1767 samples in the whole data), we further use stratified sampling so that no class remains underrepresented. We sample (without replacement) min $\{5000, \text{total number of bios data of that class}\}$ many samples from each class. We then split the data into train and test (80\% - 20\%) for model building purpose. Following table describes the number of samples from each occupation in the subsampled data: 

\begin{center}
 \begin{tabular}{|c | c | c|} 
 \hline
\textbf{Occupation} & \textbf{Male bios} & \textbf{Female Bios} \\ [0.5ex] 
\hline \hline
 Attorney & 3049 & 1951  \\ 
 Nurse & 460 & 4540  \\
 Paralegal & 268 &  1499  \\
 Physician & 2504 & 2496 \\ [1ex] 
 \hline
\end{tabular}
\end{center}

In KNN classification technique, we use leave-one-out-cross-validation technique on the train data to tune the number of optimal neighbors $k$. For every $1 \le k \le K$ (K is some large integer, which is chosen to be 100 in our experiment) and $k$ odd, we delete one training example from the data and try to predict its occupation based on the remaining data. Finally, we select $k$ with maximum accuracy.


\section{Word embedding association tests}
\label{sec:weat}

\begin{table*}[t]
\centering
\caption{Association tests code names}
\vspace{.05in}
\begin{tabular}{lc}
\toprule
FLvINS & Flowers vs. insects \citep{greenwald1998measuring}\\
INSTvWP & Instruments vs. weapons \citep{greenwald1998measuring}\\
MNTvPHS & Mental vs. physical disease \citep{monteith2011implicit}\\
EAvAA & Europ-Amer vs Afr-Amer names \citep{caliskan2017Semantics}\\
EAvAA\citep{bertrand2004Are} & Europ-Amer vs Afr-Amer names \citep{bertrand2004Are}\\
MNvFN & Male vs. female names \citep{nosek2002harvesting}\\
MTHvART & Math vs. arts \citep{nosek2002harvesting}\\
SCvART\citep{nosek2002math} & Science vs. arts \citep{nosek2002math}\\
YNGvOLD & Young vs. old people's names \citep{nosek2002harvesting}\\
\midrule
PLvUPL &  Pleasant vs. unpleasant \citep{greenwald1998measuring} \\
TMPvPRM & Temporary vs. permanent \citep{monteith2011implicit} \\
PLvUPL\citep{nosek2002harvesting} &  Pleasant vs. unpleasant \citep{nosek2002harvesting} \\
CARvFAM & Career vs. family \citep{nosek2002harvesting}\\
MTvFT & Male vs. female terms \citep{nosek2002harvesting}\\
MTvFT\citep{nosek2002math} & Male vs. female terms \citep{nosek2002math}\\
\bottomrule
\end{tabular}
\label{table:association_names}
\end{table*}



==> goku-macros.tex <==

\def\Avar{{\sf Avar}}
\def\abs#1{\left|#1\right|}
\def\aff{{\sf aff}}
\def\argmin{{\arg\min}}
\def\argmax{{\arg\max}}
\def\avar{{\sf avar}}

\def\bA{\mathbf{A}}
\def\bB{\mathbf{B}}
\def\bC{\mathbf{C}}
\def\bD{\mathbf{D}}
\def\bE{\mathbf{E}}
\def\bF{\mathbf{F}}
\def\bff{\mathbf{f}}
\def\bG{\mathbf{G}}
\def\bH{\mathbf{H}}
\def\bI{\mathbf{I}}
\def\bJ{\mathbf{J}}
\def\bK{\mathbf{K}}
\def\bL{\mathbf{L}}
\def\bM{\mathbf{M}}
\def\bN{\mathbf{N}}
\def\bO{\mathbf{O}}
\def\bP{\mathbf{P}}
\def\bQ{\mathbf{Q}}
\def\bR{\mathbf{R}}
\def\bS{\mathbf{S}}
\def\bT{\mathbf{T}}
\def\bU{\mathbf{U}}
\def\bV{\mathbf{V}}
\def\bW{\mathbf{W}}
\def\bX{\mathbf{X}}
\def\bY{\mathbf{Y}}
\def\bZ{\mathbf{Z}}

\def\bGamma{{\boldsymbol\Gamma}}
\def\bDelta{{\boldsymbol\Delta}}
\def\bTheta{{\boldsymbol\Theta}}
\def\bLambda{{\boldsymbol\Lambda}}
\def\bXi{{\boldsymbol\Xi}}
\def\bPi{{\boldsymbol\Pi}}
\def\bSigma{{\boldsymbol\Sigma}}
\def\bUps{{\boldsymbol\Upsilon}}
\def\bPhi{{\boldsymbol\Phi}}
\def\bPsi{{\boldsymbol\Psi}}
\def\bOmega{{\boldsymbol\Omega}}

\def\ba{\mathbf{a}}
\def\bb{\mathbf{b}}
\def\bc{\mathbf{c}}
\def\bbd{\mathbf{d}}
\def\bd{{\sf bd}}
\def\be{\mathbf{e}}
\def\bbf{\mathbf{f}}
\def\bg{\mathbf{g}}
\def\bh{\mathbf{h}}
\def\bi{\mathbf{i}}
\def\bj{\mathbf{j}}
\def\bk{\mathbf{k}}
\def\bl{\mathbf{l}}
% \def\bm{\mathbf{m}}
\def\bn{\mathbf{n}}
\def\bo{\mathbf{o}}
\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\br{\mathbf{r}}
\def\bs{\mathbf{s}}
\def\bt{\mathbf{t}}
\def\bu{\mathbf{u}}
\def\bv{\mathbf{v}}
\def\bw{\mathbf{w}}
\def\bx{\mathbf{x}}
\def\by{\mathbf{y}}
\def\bz{\mathbf{z}}

\def\balpha{{\boldsymbol\alpha}}
\def\bbeta{{\boldsymbol\beta}}
\def\bgamma{{\boldsymbol\gamma}}
\def\bdelta{{\boldsymbol\delta}}
\def\beps{{\boldsymbol\epsilon}}
\def\bveps{{\boldsymbol\varepsilon}}
\def\bzeta{{\boldsymbol\zeta}}
\def\bfeta{{\boldsymbol\eta}}
\def\btheta{{\boldsymbol\theta}}
\def\bvtheta{{\boldsymbol\vartheta}}
\def\biota{{\boldsymbol\iota}}
\def\bkappa{{\boldsymbol\kappa}}
\def\blambda{{\boldsymbol\lambda}}
\def\bmu{{\boldsymbol\mu}}
\def\bnu{{\boldsymbol\nu}}
\def\bxi{{\boldsymbol\xi}}
\def\bpi{{\boldsymbol\pi}}
\def\brho{{\boldsymbol\rho}}
\def\bvrho{{\boldsymbol\varrho}}
\def\bsigma{{\boldsymbol\sigma}}
\def\btau{{\boldsymbol\tau}}
\def\bups{{\boldsymbol\upsilon}}
\def\bphi{{\boldsymbol\phi}}
\def\bvphi{{\boldsymbol\varphi}}
\def\bpsi{{\boldsymbol\psi}}
\def\bomega{{\boldsymbol\omega}}

\def\bbA{\mathbb{A}}
\def\bbB{\mathbb{B}}
\def\bbC{\mathbb{C}}
\def\bbD{\mathbb{D}}
\def\bbE{\mathbb{E}}
\def\bbF{\mathbb{F}}
\def\bbG{\mathbb{G}}
\def\bbH{\mathbb{H}}
\def\bbI{\mathbb{I}}
\def\bbJ{\mathbb{J}}
\def\bbK{\mathbb{K}}
\def\bbL{\mathbb{L}}
\def\bbM{\mathbb{M}}
\def\bbN{\mathbb{N}}
\def\bbO{\mathbb{O}}
\def\bbP{\mathbb{P}}
\def\bbQ{\mathbb{Q}}
\def\bbR{\mathbb{R}}
\def\bbS{\mathbb{S}}
\def\bbT{\mathbb{T}}
\def\bbU{\mathbb{U}}
\def\bbV{\mathbb{V}}
\def\bbW{\mathbb{W}}
\def\bbX{\mathbb{X}}
\def\bbY{\mathbb{Y}}
\def\bbZ{\mathbb{Z}}

\def\Ber{{\sf Ber}}
\def\bin{{\sf bin}}

\def\cA{\mathcal{A}}
\def\cB{\mathcal{B}}
\def\cC{\mathcal{C}}
\def\cD{\mathcal{D}}
\def\cE{\mathcal{E}}
\def\cF{\mathcal{F}}
\def\cG{\mathcal{G}}
\def\cH{\mathcal{H}}
\def\cI{\mathcal{I}}
\def\cJ{\mathcal{J}}
\def\cK{\mathcal{K}}
\def\cL{\mathcal{L}}
\def\cM{\mathcal{M}}
\def\cN{\mathcal{N}}
\def\cO{\mathcal{O}}
\def\cP{\mathcal{P}}
\def\cQ{\mathcal{Q}}
\def\cR{\mathcal{R}}
\def\cS{\mathcal{S}}
\def\cT{\mathcal{T}}
\def\cU{\mathcal{U}}
\def\cV{\mathcal{V}}
\def\cW{\mathcal{W}}
\def\cX{\mathcal{X}}
\def\cY{\mathcal{Y}}
\def\cZ{\mathcal{Z}}

\def\cat{{\sf cat}}
\def\Cov{{\sf Cov}}
\def\cov{{\sf cov}}
\def\card{{\bf card}}
\def\cf{{\it cf.}}
\def\cl{{\sf cl}}
\def\complex{{\bbC}}
\def\cone{{\sf cone}}
\def\conv{{\sf conv}}
\def\deq{\overset{d}{=}}
\def\det{{\sf det}}
\def\diag{{\sf diag}}
\def\diam{{\sf diam}}
\def\dist{{\sf dist}}
\def\dom{{\sf dom}}
\def\doop{{\sf do}}
\def\dto{\overset{\sf d}{\to}}
\def\Ex{{\bbE}}
\def\Exp{{\sf Exp}}
\def\exp{{\sf exp}}
\def\eg{{\it e.g.}}
\def\epi{{\sf epi}}
\def\eps{{\epsilon}}
\def\etc{{\it etc.}}
\def\ie{{\it i.e.}}
\def\iid{{\sf iid}}
\def\ind{{\sf ind}}
\def\intr{{\sf int}}
\def\integers{{\bbZ}}

\def\halpha{\widehat{\balpha}}
\def\hbeta{\widehat{\bbeta}}
\def\hdelta{\widehat{\bdelta}}
\def\hGamma{\widehat{\bGamma}}
\def\hgamma{\widehat{\bgamma}}
\def\hmu{\widehat{\bmu}}
\def\hSigma{\widehat{\bSigma}}
\def\hsigma{\widehat{\bsigma}}
\def\hTheta{\widehat{\bTheta}}
\def\htheta{\widehat{\btheta}}
\def\hw{\widehat{\bw}}

\def\KL{{\sf KL}}
\def\ker{{\sf ker}}
\def\lspan{{\sf span}}
\def\maximize{{\sf maximize}}
\def\med{{\sf med}}
\def\minimize{{\sf minimize}}
\def\norm#1{\left\|#1\right\|}
\def\ones{\mathbf{1}}
\def\Poi{{\sf Poi}}
\def\Pr{{\bbP}}
\def\peq{\overset{\sf p}{=}}
\def\plim{{\sf plim}}
\def\proj{{\sf proj}}
\def\prox{{\sf prox}}
\def\pto{\overset{\sf p}{\to}}
\def\ran{{\sf ran}}
\def\rank{{\sf rank}}
\def\reals{{\bbR}}
\def\relint{{\sf relint}}
\def\sign{{\sf sign}}
\def\supp{{\sf supp}}
\def\symm{{\bbS}}

\def\st{\textrm{subject to}}
\def\tr{{\sf tr}}
\def\tube{{\sf tube}}
\def\TV{{\sf TV}}
\def\unif{{\sf unif}}
\def\Var{{\sf Var}}
\def\var{{\sf var}}
\def\vct{{\sf vec}}
\def\veps{\varepsilon}
\def\vol{{\sf vol}}
\def\zeros{\mathbf{0}}


==> goku-thm-macros.tex <==

\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{model}[theorem]{Model}
% \newenvironment{proof}{\noindent {\sc Proof:}}{$\Box$ \medskip} 
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}


==> proofs.tex <==
\section{Proofs}
\label{sec:proofs}

\subsection{Proof of Lemma \ref{identifiability}}
From the definition of $M(\Sigma)$ we have: 
\allowdisplaybreaks
\begin{align*}
\left\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0)) \right\rangle & = \left\langle (\Sigma - \Sigma_0), E\left[D(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle))\right]\right\rangle \\
& = E\left[\left(\langle \Sigma, D \rangle  - \langle D, \Sigma_0 \rangle\right)\left(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle)\rangle\right)\right] \\
& = E\left[\left(\langle \Sigma, D \rangle - \langle \Sigma_0, D \rangle \right)(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle))\right] \\
& \ge 0 \hspace{0.1in} [\text{As F is monotone}]
\end{align*}
Next we prove $\left\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0)) \right\rangle = 0$ implies $\Sigma = \Sigma_0$. From the monotonicity of $F$ $$\left(\langle \Sigma, D \rangle - \langle \Sigma_0, D \rangle \right)(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle)) \ge 0$$ a.s in $D$. Hence $$\left\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0)) \right\rangle = 0 \Rightarrow \left(\langle \Sigma, D \rangle - \langle \Sigma_0, D \rangle \right)(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle)) = 0$$ a.s in $D$. Assumption 3 asserts that $F$ is strictly increasing on the support of $\langle D, \Sigma \rangle$, which, in turn, indicates that $\langle \Sigma, D \rangle = \langle \Sigma_0, D \rangle$ a.s. $D$. i.e. $X'\Sigma X = X'\Sigma_0 X$ a.s. $X$. This immediately implies $\Sigma = \Sigma_0$ as the support of $X$ is not confined in any proper subspace of $\mathbb{R}^d$. 


\subsection{Proof of Theorem \ref{main_theorem}}
The consistency of our estimator follows directly from the tail bound, hence we only prove part 2 of the theorem. We break the proof into few small lemmas.
\begin{lemma}
\label{score_curvature}
Under our model assumptions we have $$\|M(\Sigma) - M(\Sigma_0)\|_F \ge \sqrt{c}\lambda_-\|\Sigma - \Sigma_0\|_F $$ for all $\Sigma \in \Theta$, where the constants $c, \lambda_-$ are as defined in the assumptions.
\end{lemma}

\begin{proof}
We prove a more general result, from which the conclusion of the Lemma will follow immediately. We show that: $$\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0))\rangle \ge \mu \|\Sigma - \Sigma_0\|^2_F$$ for some constant $\mu > 0$. Towards that end, 
\allowdisplaybreaks
\begin{align}
\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0))\rangle & = \langle (\Sigma - \Sigma_0), E\left[D(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle))\right] \rangle \notag \\
& = E\left[\left(\langle \Sigma, D \rangle  - \langle D, \Sigma_0 \rangle\right)\left(F(-\langle D, \Sigma_0 \rangle) - F(-\langle D, \Sigma \rangle)\right)\right] \notag \\
& = E\left[\left(\langle \Sigma, D \rangle  - \langle D, \Sigma_0 \rangle\right)^2f(-\langle D, \alpha\Sigma_0+(1-\alpha)\Sigma \rangle)\right] \notag \\
& \ge c E\left[\left(\langle \Sigma, D \rangle  - \langle D, \Sigma_0 \rangle\right)^2\right] \notag \\
& = c E\left[(X'(\Sigma - \Sigma_0)X)^2\right] \notag \\
& \ge c \|\Sigma - \Sigma_0\|_F^2 \left(\inf_{A \in S^d, \|A\|_F = 1} E\left[(X'AX)^2\right]\right) \notag
\end{align}
We claim that: $$\inf_{A \in S^d, \|A\|_F = 1} E\left[(X'AX)^2\right] > 0$$ We prove this by contradiction. Assume that the infimum is 0. As the infimum is taken of a continuous function over a compact set, it must be attained. Hence, there is some symmetric matrix $A_0$ such that  $E\left[(X'A_0X)^2\right] = 0$. This implies $X'A_0X = 0$ a.s. which further implies that support of $X$ is a boundary of an ellipse of $R^d$ which contradicts Assumption 2. Hence $\inf_{A \in S^d, \|A\|_F = 1} E\left[(X'AX)^2\right]  = \lambda_- > 0$ and we conclude that $$\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0))\rangle \ge c\lambda_- \|\Sigma - \Sigma _0\|_F^2$$ The conclusion of the lemma now follows from the observation 
\allowdisplaybreaks
\begin{align*}
\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0))\rangle  \le \|M(\Sigma) - M(\Sigma_0)\|_F \|\Sigma- \Sigma_0\|_F
\end{align*}
\end{proof}




\begin{lemma}
\label{grad_bound}
Under assumptions 1-3, we have with probability greater than $1 - \delta$, $$\|M(\hSigma_n) - M(\Sigma_0)\|_F \le \frac{C_0}{\sqrt{n}}+\sqrt{\frac{2U\log{\frac{2}{\delta}}}{n}}$$ for some constant $C_0$. 
\end{lemma}

\begin{proof}
We start with the following basic risk analysis: 
\allowdisplaybreaks
\begin{align*}
\|M(\hSigma) - M(\Sigma_0)\|_F = \|M_n(\hSigma) - M(\hSigma)\|_F \le \sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F
\end{align*}
Now to establish concentration of $\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F$, we break the problem two parts. We show that $$\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F - E\left(\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F\right)$$ concentrates and $E\left(\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F\right)$ concentrates. For the first part, we use Mcdiarmid's inequality. Define $$g((y_1, x_1), \dots, (y_n, x_n)) = \sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F$$ Now if we replace one sample $(x_i, y_i)$ by another copy of $(x'_i, y'_i)$ then the maximum fluctuation of the function $g$ can be bounded as below: 
\allowdisplaybreaks
\begin{align*}
& \left|g((y_1, x_1), \dots, (y_i, x_i), \dots, (y_n, x_n))  - g((y_1, x_1), \dots, (y_i', x_i'), \dots, (y_n, x_n))\right| \\
& \le \sup_{\Sigma \in \Theta} \frac{2}{n} \left\|D_i(y_i - F(-\vc(\Sigma)'\vc(D_i)))  -D'_i(y'_i - F(-\vc(\Sigma)'\vc(D'_i)))\right\|_F \\
& \le \frac{4U^2}{n} 
\end{align*}
Using Mcdiarmid's inequality we can conclude: 
\allowdisplaybreaks
\begin{align*}
P\left(\left|Z - EZ\right| \ge t\right) \le 2e^{-\frac{nt^2}{2U^2}}
\end{align*} 
where $Z = \sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F$. Hence with probability $\ge 1-\delta$, we have: 
\begin{equation}
\label{varscore}Z \le EZ + \sqrt{\frac{2U\log{\frac{2}{\delta}}}{n}}
\end{equation}
For the concentration of $E\left(\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|\right)$ we borrow some existing bound ideas from empirical process theory. Observe that 


\begin{align*}
E\left(\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F\right) & = E\left(\sup_{\Sigma \in \Theta} \|M_n(\vc(\Sigma)) - M(\vc(\Sigma))\|_2\right) \\
& = E\left(\sup_{\Sigma \in \Theta}\sup_{v: \|v\| \le 1} \langle v,  M_n(\vc(\Sigma)) - M(\vc(\Sigma)) \rangle \right) \\
& = E\left(\sup_{g_{\Sigma, v} \in \mathcal{G}} (P_n - P)(h_{\vc(\Sigma), v})\right)
\end{align*}
where $$h_{\vc(\Sigma),v}(X,Y) = (v'\vc(D))(Y - F(-\vc(D)'\Sigma))$$ and $\mathcal{H} = \{h_{\Sigma, v}: \Sigma \in \Theta, \|v\|_2 \le 1\}$. It is immediate that VC dimension of class of functions $\mathcal{H}$ is finite. Using this we conclude that, there exists some constant $C_0$ such that: 


\begin{equation}
\label{exscore} E\left(\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\|_F\right) \le \frac{C_0}{\sqrt{n}}
\end{equation}

\noindent
Combining equation \ref{varscore} with \ref{exscore} we conclude that with probability $\ge 1-\delta$ we have: 

\begin{equation}
\sup_{\Sigma \in \Theta} \|M_n(\Sigma) - M(\Sigma)\| \le \frac{C_0}{\sqrt{n}} + \sqrt{\frac{2U\log{\frac{2}{\delta}}}{n}}
\end{equation}
which concludes the proof.
\end{proof}
Finally, combining Lemma \ref{score_curvature} and \ref{grad_bound} we get with probability greater than $1 - \delta$: 
\allowdisplaybreaks
\begin{align*}
\|\hSigma - \Sigma\|_F  & \le \frac{1}{\sqrt{c}\lambda_-}\|M(\hSigma) - M(\Sigma_0)\|_F \hspace{0.1in} [\text{Lemma} \  \ref{score_curvature}]\\
& \le \frac{C_0}{\sqrt{c}\lambda_-\sqrt{n}}+\sqrt{\frac{2U\log{\frac{2}{\delta}}}{c\lambda^2_-n}}  \hspace{0.1in} [\text{Lemma} \  \ref{grad_bound}]
\end{align*}
Taking $b = \frac{C*0}{\sqrt{c}\lambda_-}$ and $a = \frac{c\lambda^2_-}{2U}$, we conclude the tail bound. 
\\\\

Finally we prove part 3 of the theorem. We first show that the log-likelihood function has quadratic upper bound, i.e.: 
$$\ell(\Sigma_0) - \ell(\Sigma) \lesssim \|\Sigma - \Sigma_0\|^2_F$$ Recall that the log-likelihood function is defined as: 
\allowdisplaybreaks
\begin{align*}
\ell(\Sigma) & = E\left[Y\log\frac{F(\langle D,\Sigma\rangle)}{1-F(\langle D,\Sigma\rangle)} + (\log(1-F(\langle D,\Sigma\rangle))\right] \\
& =  E\left[F(\langle D, \Sigma_0 \rangle)\log\frac{F(\langle D,\Sigma\rangle)}{1-F(\langle D,\Sigma\rangle)} + (\log(1-F(\langle D,\Sigma\rangle))\right] \\
& =  E\left[F(\langle D, \Sigma_0 \rangle)\log{F(\langle D,\Sigma\rangle)} + (1-F(\langle D,\Sigma_0\rangle))\log{(1-F(\langle D,\Sigma\rangle))}\right] \\
& = \ell(\Sigma_0) - E\left[KL\left(Ber(F(\langle D, \Sigma_0 \rangle)) \ || \ Ber(F(\langle D, \Sigma \rangle))\right)\right]
\end{align*}



==> rebuttal.tex <==
We thank the reviewers for their time and encouraging feedback. Please find the individual responses below.

R3: We thank the reviewer for positive feedback and for pointing out the typos. We will revise accordingly.

R4: Comparison with methods like LMNN: We thank the reviewer for pointing us to LMNN and related methods. While it is certainly possible to adapt these methods for fair metric learning from pair-wise comparisons (the setting of EXPLORE), they are not immediately applicable because their main goal is improving the accuracy of K-nearest neighbors classifiers. For example, unlike EXPLORE, LMNN requires the user to specify a set of K possible neighbors for each training example and learns a metric that separates this set of possible neighbors from the rest of the training examples. As you mentioned in your comments, these LMNN-type methods also lack statistical guarantees because they are not motivated by a probabilistic model of the data. Nevertheless, studying LMNN-type methods for fair metric learning is a promising direction for future work. For example, it may be possible to simultaneously incorporate human feedback in the forms of comparable groups and pair-wise comparisons with an LMNN-type methods. We will add a discussion of LMNN-type methods in a revised version.

R4: Comparison with Ilvento's work: We mention Ilvento because she considers the same task of fair metric learning, but her setting is different from ours. In our setting, the human feedback consists of either groups of comparable samples or pair-wise comparisons between samples. In her setting, the human feedback consists of (possibly noisy) real-valued distances between samples or relative comparisons of the form X_1 is closer to X_2 than it is to X_3. We did not include her methods as baselines because her setting is not suitable for the applications that we considered. We will clarify this in the paper.

R5: Connection between algorithm and theory: Section 3.2 exactly analyzes the FACE algorithm as described in Section 2.1. The connection between the intuition behind FACE and the assumptions of Theorem 3.2 may have been lost because we dropped a mean term from the right side of the equation in line 223(left). Although this does not affect the rest of the theoretical developments (i.e. no loss of generality), we see how it could make it harder to connect algorithm and the theory. 

All the individuals in a comparable group of samples have similar relevant factors, so the effect of the relevant factors appear in the mean structure of a comparable group. We emphasize here that this is only the case for a comparable group; the relevant factors differ among incomparable individuals, so the effect of the relevant factors appear in the variance structure. The centering/de-meaning step in FACE is crucial because it removes the effect of the relevant attributes. Returning to the equation in line 223 (left), the B_*\nu_i term actually captures the effects of residual variation in relevant factors because the relevant factors, while similar, may not be exactly equal in a comparable group (the ``main'' effect of the relevant factors is captured by the mean term). Thus the intuition that all individuals in a comparable group have similar relevant factors translates into small residual variation in the relevant factors within a comparable group, which justifies the assumption on the smallness of B_*. 

R5: Why do you take gender into account while defining comparable groups? -- In this experiment, we use gender to define comparable groups out of convenience. Gender information is available in the data set and pairs of individuals with opposite gender provide meaningful variation for learning the fair metric with EXPLORE. We emphasize that our method does not require access to the sensitive attribute information, but, if this information is available, then it is one way to obtain comparable groups without the need to collect additional data. 

R5: Evaluation metrics -- we chose Gaps as group fairness metrics following prior works, however we note that spouse consistency and GR consistency are notions of individual fairness. They measure (the inverse of) how many times a classifier changes its prediction on an individual when a corresponding attribute is modified. For example, if an unmarried person is predicted as low income, while a married person with same work experience is predicted high income, it is a violation of individual fairness. We will clarify the comparison metrics and also add baseline descriptions as you suggested.

R5: By isotropic, we mean the covariance matrix is the identity. This is an identification restriction, so it does not restrict the expressivity of the model: we can always include a factor of \Sigma_{\nu}^{1/2} in  A_* and B_*.

R5: The generalization result in Yurochkin et al depends on the error in the learned fair metric. Theorem 3.3 is a combination of our results on the error in the fair metric (Thm 3.2) and the generalization results in Yurochkin et al.



==== STUFF THAT WAS CUT ====


We emphasize that the assumption that A_* is larger than B_* is crucial: if there is no variation in the comparable groups due to the sensitive/protected factors, then it is impossible to learn how the individuals vary as the sensitive/protected factors vary.

Learning a fair metric automatically, i.e. not requiring any prior knowledge of the problem (or human feedback) could be very challenging if at all possible (after all, mathematically any type of fairness is a constraint that needs to be communicated to the algorithm is some way). In this specific experiment, simply sampling from the same class will introduce a lot of noise (because males are the majority in the >50k class in this dataset) and could reduce the quality of the EXPLORE fair metric.


One last point we want to clarify is that the population covariance matrix of the observations in a comparable group is denoted by Sigma_phi (line 240-241 left column) and the orientation matrix for our fair metric is defined by Sigma_0 (line 170, right column). Our estimator Sigma_hat estimates Sigma_0, not Sigma_phi (Theorem 3.2). 
    

==> statisticalTheory.tex <==
\subsection{Statistical properties}
%In this section we describe some statistical properties of our learning algorithm. Recall that, we are not exactly solving the maximum likelihood equation, due to potential non-convexity even under known link function. Instead we resort to a score equation which we show to have good statistical and computational guarantees. The score function to estimate the weight matrix $\Sigma$ for known link function is defined as $$\psi_n(\Sigma) = \frac{1}{n} \sum_{i=1}^n D_i (y_i -  F(-\langle D_i, \Sigma \rangle))$$ where $\langle . \rangle$ is the Frobenious inner product of matrices. For unknown link, we use isotonic estimate of $F$ in the score function: $$\tilde{\psi}_n(\Sigma) = \frac{1}{n} \sum_{i=1}^n D_i (y_i -  \hat F_{\Sigma}(-\langle D_i, \Sigma \rangle))$$ Here we do the isotonic regression based on $\{(y_i, -\langle D_i, \Sigma \rangle)\}_{i=1, \dots, n}$ to get an estimate of $\hat F_{\Sigma}$. To establish statistical properties of the solution of the score equation, under known link function, we need the following assumptions: 

In this section we establish some statistical properties of $\hSigma$. The population version of the score function can be defined as: $$M(\Sigma) = E\left[D(y - F_0(-\langle D, \Sigma \rangle))\right]$$ where $D = XX'$. First, we show that our model is identifiable under known link function, then we establish consistency and finite sample concentration guarantees of the score estimator. Define a function $\vc(A)$ on the set symmetric matrices which vectorizes the matrix. Note that, $\|A\|_F = \|\vc(A)\|_2$. Before going into the theoretical results, we articulate our assumptions below:

\begin{assumption}
The observation $X \sim P$ for some distribution on $\mathbb{R}^d$ and has a compact support i.e., $\|X\|_2 \le U$ a.s. for some $U < \infty$. $Y$ is binary response with $P(Y=1|X) = F_0(- \langle D, \Sigma_0 \rangle)$ with $D \equiv XX'$. The support of $X$ is not confined in any proper subspace of $\mathbb{R}^{d}$ and it has non-null interior. 
\end{assumption}


\begin{assumption} 
Our parameter space is $\Theta \subset S_+^d$ has bounded operator norm, i.e., there exits $\lambda_{max} < \infty$, such that $\|\Sigma\|_{op} \le \lambda_{max}$ for all $\Sigma \in \Theta$. ({\bf Probably we don't need it.})
\end{assumption}

\begin{assumption}
The link function $F_0$ is absolutely continuous with density $f$ and $f(t) \le C < \infty$ for all $t$, $f(t) \ge c > 0$ for all $t \in (-2\lambda_{max}U^2, 0)$. 
\end{assumption}
 
The following lemma establishes the identifiability of the parameter of interest under known link function assumption: 
\begin{lemma}
\label{identifiability}
Under our model assumptions, we have $$\left\langle (\Sigma - \Sigma_0), (M(\Sigma) - M(\Sigma_0)) \right\rangle \ge 0$$ for all $\Sigma \in \Theta$ and equality holds iff $\Sigma = \Sigma_0$. 
\end{lemma}  
Next we show that the true $\Sigma_0$ satisfies variational inequality uniquely. The following theorem establishes some statistical guarantees of our estimator: 
\begin{theorem}
\label{main_theorem}
Suppose link function $F_0$ is known and $\hSigma_n$ to be root of the score function $M_n(\Sigma)$ as defined in the previous section. Then under above assumptions: 
\begin{enumerate}
\item The root is a consistent estimator, i.e., $\hSigma_n \overset{P} \longrightarrow \Sigma_0$.
\item The root has sub-gaussian tail concentration, i.e. there exists constant $a,b$ such that $$P(\sqrt{n}\|\hSigma - \Sigma_0\| \ge t) \le 2e^{-a(t -b)^2}$$. 
\end{enumerate}
\end{theorem}



==> theory.tex <==
\section{Theoretical properties of EXPLORE and FACE}
\label{sec:theory}

In this section, we investigate the theoretical properties of FACE and EXPLORE. We defer proofs to Appendix \ref{sec:proofs}.
\DM{we need to decide which part of the theory should stay here and which part will go to the appendix.}
\subsection{Theoretical properties of EXPLORE}
\label{sec:logisticTheory}
We provide statistical guarantees corresponding to the estimation using the scaled logistic link (Section \ref{matrix-logistic}). To keep things simple, we tweak \eqref{eq:binaryResponseModel} so that it is strongly identifiable:
\[
y_i\mid z_{i_1},z_{i_2} \sim \Ber((2-\eps)\sigma(-\langle D_i,\Sigma_0\rangle))
\]
for some small $\eps > 0$. The log-likelihood of samples $(x_1,y_1),\dots,(x_n,y_n)$ is 
\allowdisplaybreaks
\begin{align*}
    \ell_n(\Sigma) &\textstyle = \frac1n \sum_{i=1}^n \left[y_i \log{F_*(x_i'\Sigma x_i)} \right. \\
    & \qquad \qquad \qquad \left. + (1-y_i) \log{(1 - F_*(x_i'\Sigma x_i))}\right],
\end{align*}
where $F_* = (2-\epsilon)\sigma$. 

\begin{lemma}
\label{convexity}
The population version of the likelihood function $\ell(\Sigma)$ is concave in $\Sigma$ and uniquely maximized at $\Sigma_0$. 
\end{lemma}

% For theoretical simplicity, assume that the model is $$P(Y=1|X=x) = (2-\epsilon)\sigma(x'\Sigma_0 x)$$ for some $\epsilon > 0$ fixed. This minute modification makes the likelihood function bounded and theoretically more amenable. \footnote{However, it is certainly possible to extend the analysis without this modification at the cost of substantially more tedious calculation.}We state the new model below: 
% \allowdisplaybreaks
% \begin{align*}
%     & \qquad  \qquad X \sim P \\
%     & P(Y=1|X=x) = (2 - \epsilon)\sigma(x'\Sigma_0 x) = \frac{2-\epsilon}{1+e^{x'\Sigma_0 x}}\,.
% \end{align*}
% For notational simplicity, define $F_* = (2-\epsilon)\sigma$. We have i.i.d. observations $\{x_i, y_i\}_{i \in \{1,2, \dots, n\}}$ from this model where $x_i = \varphi_{i_1} - \varphi_{i_2}$. The empirical likelihood function based on the observations is:
% \allowdisplaybreaks
% \begin{align*}
%     \ell_n(\Sigma) & = \frac1n \sum_{i=1}^n \left[y_i \log{F_*(x_i'\Sigma x_i)} \right. \\
%     & \qquad \qquad \qquad \left. + (1-y_i) \log{(1 - F_*(x_i'\Sigma x_i))}\right],
% \end{align*}
% and the corresponding population version is: 
% \allowdisplaybreaks
% \begin{align*}
%     \ell(\Sigma) & = E\left[Y \log{F_*(X'\Sigma X)} + \right. \\
%     & \qquad \qquad \qquad \left. (1-Y) \log{(1 - F_*(X'\Sigma X))}\right]
% \end{align*}

% \noindent
% The following lemma proves that the population version is concave in $\Sigma$ and has a unique maximizer at $\Sigma_0$:
% \begin{lemma}
% \label{convexity}
% The population version of the likelihood function $\ell(\Sigma)$ is concave in $\Sigma$ and uniquely maximized at $\Sigma_0$. 
% \end{lemma}

The maximum likelihood estimator (MLE) $\hSigma$ is $$\hSigma = \argmax_{\Sigma} \ell_n(\Sigma)$$ 
The asymptotic properties of $\hSigma$ (consistency and asymptotic normality) are well-established in the statistical literature (e.g. see \citet{vandervaart1998Asymptotic}). Here we study the non-asymptotic convergence rate of the MLE. We start by stating our assumptions.

\begin{assumption}
\label{Sample_space}
The feature space $\mathcal{X}$ is a bounded subset of $\mathbb{R}^d$, \ie\ there exits $U < \infty$ such that $\|X\| = \|\varphi_1 - \varphi_2\| \le U$ for all $X \in \mathcal{X}$. 
\end{assumption}

\begin{assumption}
\label{parameter_space}
The parameter space $\Theta$ is a subset of $\mathbb{S}_{++}^d$ and $\sup\{\lambda_{max}(\Sigma):\Sigma\in\Theta\} \le C_+ < \infty$.
\end{assumption}

\noindent
Under these assumptions, we establish a finite sample concentration result for our estimator $\hSigma$: 

\begin{theorem}
\label{concentration}
Under assumptions \ref{Sample_space} and \ref{parameter_space} we have the following tail bound on the estimation error: $$P(\sqrt{n} \|\hSigma - \Sigma_0\|_{op} \ge t) \le e^{-bt^2}$$ for some constant $b > 0$. 
\end{theorem}
We can combine Theorem \ref{concentration} with Proposition 3.1 of \cite{yurochkin2020Training} to show that EXPLORE in conjunction with SENSR trains individually fair ML models. Define $\mathcal{L} = \{\ell(\cdot, \theta) \ : \ \theta \in \Theta \}$ as the loss class. We assume the loss is bounded, so $0 \le \ell(z, \theta) \le M$ for all $z \in \mathcal{Z}$ and $\theta \in \Theta$, and $L$-Lipschitz with respect to $d_x$: 
\begin{align*}
    & \textstyle\sup_{\theta \in \Theta}\left\{\sup_{(x_1, y), (x_2, y)\in \mathcal{Z}}\left|\ell((x_1, y), \theta) - \ell((x_2, y), \theta)\right|\right\} \\
    & \qquad \qquad \le Ld_x(x_1, x_2);
\end{align*}
Also define $\delta_n$ to be the excess risk: 
\begin{align*}
    &\textstyle \delta_n \overset{\Delta}{=} \sup_{\theta \in \Theta} \left\{\left| \sup_{P:W_0(P, P_n) \le \epsilon} \E_P\left[\ell(Z, \theta)\right] \right. \right. \\
    &\textstyle \qquad \qquad \qquad\left. \left. - \sup_{P:W(P, P_n) \le \epsilon} \E_P\left[\ell(Z, \theta)\right]\right| \right\}
\end{align*}
where $W_*$ is the Wasserstein distance with respect to the true matrix $\Sigma_0$ and $W$ is Wasserstein distance with respect to $\hat \Sigma$. 
\begin{corollary}
\label{concentration_cor}
Using the above definitions of $\delta_n$ and assuming the loss function $\ell \in \mathcal{L}$ we have with probability $\ge 1 - t-e^{-bt^2}$: 
\begin{align*}
\delta_n &\textstyle \le \frac{48\mathcal{C}(\mathcal{L})}{\sqrt{n}} + \frac{48LU^2}{\sqrt{n}\epsilon} + \frac{LU^2t}{\sqrt{n}\lambda_{\min}(\Sigma_0)\sqrt{\epsilon}}+M\left(\frac{\log{(2/t)}}{2n}\right)^{1/2}
\end{align*}
\end{corollary}

\subsection{Theoretical properties of FACE}
\label{sec:factorAnalysisTheory}

In this section we provide some theoretical guarantees for the factor analysis based approach for the pairwise comparison model.  Define, as before, $x_i = \varphi_{i_1} - \varphi_{i_2}$, and consider only those $x_i$'s which come from a comparable pair, i.e., with corresponding $y_i = 1$. We model $x_i$ with the following simplified version of the factor model:
\begin{align}
  x_i & = \varphi_{i_1}-\varphi_{i_2} \notag\\
  & = A_*(u_{i_1}-u_{i_2}) + B_*(v_{i_1}-v_{i_2}) + (\epsilon_{i_1} - \epsilon_{i_2}) \notag\\
    \label{model_equation}   & = A_* \mu_i + B_* \nu_i + w_i
\end{align}
using the notation from Section \ref{sec:factorAnalysis}.
We assume that the sensitive attributes have more than one dimension which corresponds to the setting of \emph{intersectional fairness} (\eg\ we wish to mitigate gender and racial bias). We also assume $\mu_i$'s and $\nu_i$'s are isotropic, variance of $w_i$ is $\sigma^2I_d$ and $\mu_i, \nu_i, w_i$ are all independent of each other. The scalings of $\mu_i$ and $\nu_i$ are taken care of by the matrices $A_*$ and $B_*$ respectively. Let $\Sigma$ be covariance matrix of $x_i$. From model equation \ref{model_equation} and aforementioned assumptions: 
\begin{equation}
    \label{factor_variance}\Sigma = A_*A_*^T + B_*B_*^T + \sigma^2 I_d
\end{equation}
We assume that we know the dimension of the sensitive direction beforehand which is denoted by $k$ here. As $\phi_{i_1}$ is comparable to $\phi_{i_2}$, we expect that variability along the protected attribute is dominant. Mathematically speaking, we assume $\lambda_{min}(A_* A_*^T) > \|B_*B_*^T + \sigma^2 I_d\|_{op}$. To estimate (and hence eliminate) the effect of the protected attribute, we compute the SVD of the sample covariance matrix ($S_n$) of the $x_i$'s and project out the eigenspace corresponding to the top k eigenvectors, which we denote by $\hat U$. The following theorem quantifies the statistical error of the estimator: 
\begin{theorem}
\label{thm:svd_theorem_new}
Suppose $x_i$'s are centered sub-gaussian random vectors, i.e. $\|x_i\|_{\psi_2} < \infty$ where $\psi_2$ is the Orlicz-2 norm. Then we have: 
\allowdisplaybreaks
\begin{equation}
\begin{aligned}
    &\textstyle P\left(\|\hat U \hat U^T - \tilde{A}_*\tilde{A}_*^T\|_{op} > b + \frac{\delta \vee \delta^2}{\tilde{\gamma} - (\delta \vee \delta^2)}\right) \le 2e^{-ct^2}
\end{aligned}
\label{eq:svd_theorem_new}
\end{equation}
for all $t < (\sqrt{n}\tilde{\gamma} - C\sqrt{d}) \wedge (\sqrt{n\tilde{\gamma}} - C\sqrt{d})$, where: 
\begin{enumerate}
\item  $\tilde{A}_*$ is the collection of the eigenvectors of $A_*$.  
    \item $b = \left(\frac{\lambda_{min}(A_*A_*^T)}{\|B_*B_*^T + \sigma^2 I_d\|_{op}}-1\right)^{-1}$
 
    \item $\delta = \frac{C\sqrt{d} + t}{\sqrt{n}}$. 
    \item $\tilde{\gamma} = \lambda_{min}(A_*A_*^T) - \|B_* B_*^T\|_{op}$.
\end{enumerate}{}
The constants $C,c$ depend only on $\|x_i\|_{\psi_2}$, the Orlicz-2 norm of the $x_i$'s.
\end{theorem}

The error bound on the right side of \eqref{eq:svd_theorem_new} consists of two terms. The first term $\bar{B}$ is the approximation error/bias in the estimate of the sensitive subspace due to heterogeneity in the similar pairs. Inspecting the form of $\bar{B}$ reveals that the bias depends on the relative sizes of the variation in the sensitive subspace and that in the relevant subspace: the larger the variation in the sensitive subspace relative to that in the relevant subspace, the smaller the bias. In the ideal scenario where there is no variation in the relevant subspace, Theorem \ref{thm:svd_theorem_new} implies our estimator converges to the sensitive subspace. The second term is the estimation error, which vanishes at the usual $\frac{1}{\sqrt{n}}$-rate. In light of our assumptions on the sub-Gaussianity of the $x_i$'s, this rate is unsurprising. Finally, as mentioned in Section \ref{sec:dataDrivenMetric}, we can take our distance metric to be: 
$$d_x(x_1, x_2) = (x_1-x_2)^{\top}\hat \Sigma(x_1 - x_2) \,,$$
where $\hat \Sigma = \left(I - \hat U \hat U^{\top}\right)$. 


\subsubsection{Learning from Groupwise comparison}
In this section, we assume that we have a group of $n$ observations, who are close to each other expect for the protected attributes. We can model our observations as follows: $$\varphi_i = A_*\mu_i + B_*\nu_i + \epsilon_i \ \ \ i = 1, 2, \dots, n$$
Here, as before, $\mu_i$ represents the effect towards the sensitive direction, $\nu_i$ represents the effect towards other directions and $\epsilon_i$ is random noise. As before, we assume $\mu_i,\nu_i$'s are isotropic, $\Var(\epsilon_i) = \sigma^2I_d$ and the scale factors of $\mu_i$'s and $\nu_i$'s are taken care of by the matrices $A_*$ and $B_*$ respectively. As the relevant factors of the observations in this group are fairly close to each other, it is reasonable to assume $\var(B_*\nu_i) \approx 0$, i.e.  $\|B_*B_*\|_{op} \approx 0$. Hence to remove the effect of protected attributes, we estimate the column space of $A_*$ from the sample and then project it out. As $\Var(\nu_i)$ is small, it is reasonable to assume that, top-$k$ eigenvectors of $\Sigma_{\varphi}$ (the directions with most variablity) are mainly due to $A_*\mu_i$. Lets assume for simplicity $\Var(\mu_i) = I_k$ and $\Var(\epsilon_i) = \sigma^2 I_d$. We estimate the column space of $A_*$ by the top-$k$ eigenvectors of the sample covariance matrix $S_n$ of $\varphi_i$'s. The following theorem provides a finite sample concentration bound on the estimation error: 

\begin{theorem}
\label{thm:groupSVD}
Let $U$ (respectively $\hat U$) denote the $\mathbb{R}^{d \times k}$ matrix consisting of the top - $k$ eigenvectors of $\Sigma_{\varphi}$ (respectively $S_n$). Assume that $\varphi_i$ have subgaussian tail, i.e .$\|\varphi_i\|_{\psi_2} < \infty$. Then with probability $\ge 1 - 2e^{-ct^2}$ we have: 
    $$\textstyle\|\hat U \hat U^T - \tilde{A}_* \tilde{A}_*^T\|_{op} \le b + \frac{\delta \vee \delta^2}{\tilde{\gamma} - (\delta \vee \delta^2)} + \frac{t}{n}$$ for all $t<(\sqrt{n}\tilde{\gamma} - C\sqrt{d}) \wedge (\sqrt{n\tilde{\gamma}} - C\sqrt{d})$ where: 
\begin{enumerate}
\item  $\tilde{A}_*$ is the collection of the eigenvectors of $A_*$. 
    \item $b = \left(\frac{\lambda_{min}(A_*A_*^T)}{\|B_*B_*^T + \sigma^2 I_d\|_{op}}-1\right)^{-1}$
 
    \item $\delta = \frac{C\sqrt{d} + t}{\sqrt{n}}$. 
    \item $\tilde{\gamma} = \lambda_{min}(A_*A_*^T) - \|B_* B_*^T\|_{op}$.
\end{enumerate}{}
The constants $C,c$ only depend on the subgaussian norm constant of $\phi_i$. 
\end{theorem}

The error bound provided by Theorem \ref{thm:groupSVD} is similar to the error bound provided by Theorem \ref{thm:svd_theorem_new} consists of two terms. The first term $\bar{B}$ is again the approximation error/bias in the estimate of the sensitive subspace due to heterogeneity in the group; it has the same form as the bias as in Theorem \ref{thm:svd_theorem_new} and has a similar interpretation. The second term is the estimation error, which is also similar to the estimation error term in Theorem \ref{thm:svd_theorem_new}. The third term is the error incurred in estimating the mean of the $\varphi_i$'s. It is a higher order term and does not affect the rate of convergence of the estimator. As before our estimated fair metric will be: 
$$d_x(x_1, x_2) = (x_1-x_2)^{\top}\hat \Sigma(x_1 - x_2) \,,$$
where $\hat \Sigma = \left(I - \hat U \hat U^{\top}\right)$.

Along the same line of discussion at the end of Theorem \ref{concentration} we can combine Theorem \ref{thm:svd_theorem_new} (or Theorem \ref{thm:groupSVD}) to Proposition 3.1 of \cite{yurochkin2020Training} to get the following concentration bound on the excess risk: 
\begin{corollary}
Using the same notation as in Corollary \ref{concentration_cor} we have with probability $\ge 1-t-e^{-bt^2}$: 
\begin{align*}
\delta_n &\textstyle \le \frac{48\mathcal{C}(\mathcal{L})}{\sqrt{n}} + \frac{48LU^2}{\sqrt{n}\epsilon} \\
&\textstyle \qquad \qquad + \frac{LU^2t}{\sqrt{n}\lambda_{\min}(\Sigma_0)\sqrt{\epsilon}}+M\left(\frac{\log{(2/t)}}{2n}\right)^{1/2}
\end{align*}
\end{corollary}
% \yk{separate this result into two theorems, one at the population level, and one showing the finite-sample estimation error}
